Causal Unit Selection using Tractable Arithmetic Circuits

The unit selection problem aims to find objects, called units, that optimize a causal objective function which describes the objects' behavior in a causal context (e.g., selecting customers who are about to churn but would most likely change their mind if encouraged). While early studies focused mainly on bounding a specific class of counterfactual objective functions using data, more recent work allows one to find optimal units exactly by reducing the causal objective to a classical objective on a meta-model, and then applying a variant of the classical Variable Elimination (VE) algorithm to the meta-model -- assuming a fully specified causal model is available. In practice, however, finding optimal units using this approach can be very expensive because the used VE algorithm must be exponential in the constrained treewidth of the meta-model, which is larger and denser than the original model. We address this computational challenge by introducing a new approach for unit selection that is not necessarily limited by the constrained treewidth. This is done through compiling the meta-model into a special class of tractable arithmetic circuits that allows the computation of optimal units in time linear in the circuit size. We finally present empirical results on random causal models that show order-of-magnitude speedups based on the proposed method for solving unit selection.

==> UnitSelect.tex <==
We next review the reduction from the unit selection problem to the Reverse-MAP problem using an objective model, and the computation of Reverse-MAP by variable elimination. We slightly improve the objective model so that it now can represent causal objective function with non-root units.

Consider a structural causal model $G$, unit variables $\U$, and a causal objective function $L(\u)$ of the following form:
\begin{equation}
    \max_{\u} L(\u) = \sum_{i=1}^n w_i\cdot\pr(\y^i_{\x^i},\w^i_{\v^i}|\e^i, \u) \quad \text{where \ } w_i \geq 0 
    % \text{ \ and \ }\sum_{i=1}^n w_i = 1
    \label{eqn:objective-function}
\end{equation}
The objective $L$ is a linear combination of counterfactual probabilities \(\pr({\y^i}_{\x^i},{\w^i}_{\v^i}|\e^i, \u)\), where $\Y^i\W^i$ are outcomes, $\X^i\V^i$ are treatments, and $\E^i$ are evidence. Its semantics is: given that $(\e^i, \u)$ is observed, what is the probability that $\Y^i = \y_i$ if we $\DO(\X^i=\x^i)$, and $\W^i = \w_i$ if we $\DO(\V^i=\v^i)$. This setting is motivated by the benefit function proposed by~\cite{ijcai/LiP19} whose initial goal is to select customer characteristics $\u$ to maximize the overall benefit given the pattern of always-takers \haiying{$(y_x,  y_{x'})$}, responders \haiying{$(y_x,  y_{x'}')$}, deniers \haiying{$(y'_x,  y_{x'}')$}, and contrarians \haiying{$(y'_x,  y_{x'})$} among population group $\u$:
\begin{align}
     L(u) &= 
     \beta \pr(y_x,  y_{x'}'|\u) +  
     \gamma\pr(y_x,  y_{x'}|\u) \nonumber \\ 
     &\quad +\theta\pr(y_x', y_{x'}'|\u) + 
     \delta\pr(y_x', y_{x'}|\u)
     \label{eqn:benefit-ang}
\end{align}
\haiying{
Here, $(\beta, \gamma, \theta, \delta)$ are the benefits of selecting one individual of each type respectively, and the objective function $L$ is the average benefit gained from a specific population group $\u$.
}

The treatment in~\cite{huang2023algorithm} generalizes this problem to (almost) any causal objective function $L$ that can be expressed as a linear combination of counterfactual, interventional, or classical probabilities. They provide a principled way to reduce this type of objective function to a single observational probability on an objective model. This leads to many benefits. For example, each component $\pr^i$ can have multiple variables for treatments $\X^i,\V^i$ and they can be different across $i$; multiple variables for outcomes $\Y^i,\W^i$ and they can be different across $i$; there can be many unit variables $\U$ so it poses a computational challenge. We next review the construction of the objective model
in~\cite{huang2023algorithm}
while lifting their restriction that unit variables must be exogenous (roots).

\paragraph{Objective Model} Consider an SCM $G$ with unit variables $\U$. The construction of the objective model has two steps: reduce and compose. The first step is to reduce each counterfactual component \(\pr({\y^i}_{\x^i},{\w^i}_{\v^i}|\e^i, \u)\) to an observational probability on a triplet model $G^i$. This is done by creating 3 copies\footnote{We need 3 copies as $G$ is for the real-world, $[G]$ is for event ${\y^i}_{\x^i}$, and $[[G]]$ is for event ${\w^i}_{\v^i}$.} of $G$, denoted by $G$, $[G]$, $[[G]]$ and join them so that they share all exogenous variables. We remove edges pointing into intervened variables $\X^i$, $\V^i$ in copies $[G]$, $[[G]]$ respectively. The counterfactual probability is then reduced to a classical one $\pr([\y^i], [[\w^i]] \cond [\x^i], [[\v^i]], \e^i, \u)$ on $G^i$. We point out that this is based on a standard technique known as twin-networks~\cite{aaai/BalkeP94}. 

Given a list of triplet models $G^1,\ldots, G^n$ and each $\pr^i$ has the form of a classical probability. The second step is to combine $(G^i, \pr^i)$ such that the linear combination $\sum \pr^i$ is reduced to a single classical probability. As~\cite{huang2023algorithm} shows, this can be achieved by adding a mixture node as a common parent of outcome nodes and ``syncing" unit nodes $\U$ among $G^i$.

\begin{figure*}[t]
    \centering
\begin{subfigure}{0.1\textwidth}
    \includegraphics[width=\textwidth]{figures/base.png}
    \caption{SCM}
    \label{fig:scm}
\end{subfigure}
\hspace{1cm} % Spacing between the subfigures
\begin{subfigure}[b]{0.2\textwidth}
    \includegraphics[width=\textwidth]{figures/mut-triplet2.png}
    \caption{triplet model (intervened)}
    \label{fig:triplet}
\end{subfigure}
\hspace{1cm} % Spacing between the subfigures
\begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{figures/objective2.png}
    \caption{objective model}
    \label{fig:objective}
\end{subfigure}

\caption{Example showing the obective model for a causal objective function with 2 components (Huang and Darwiche 2023).}
\label{fig:test}
\end{figure*}

\begin{definition}[Objective Model]
\label{def:objective model}
Consider an SCM $G$ and
the objective function $L$ in Equation~\ref{eqn:objective-function}.
Let $\U^r \subseteq \U$ be the subset of $\U$ that is root and $\U^c$ be the subset that is internal.
The objective model $G’$ for 
$\langle G,L\rangle$ is constructed as follows:
\begin{enumerate}
\item Construct a triplet model $G^i$ of $G$ for each term $\pr^i(\y^i_{\x^i}, \w^i_{\v^i}|\e^i, \u)$ in $L$. 
\item Join  $G_1, G_2, \ldots, G_n$ such that $\U^r$ are shared and for each $U \in \U^c$, add an auxiliary node $\Lambda_U$ as a common child of nodes  $\{U^i\}$. $\Lambda_U$ is binary and its CPT is set so that $\Lambda_U = 1$ iff $\{U^i\}$ take consistent values.
\item Add a node $H$ to \(G'\) as a parent of all outcome nodes $\Z = \{[\Y^i], [[\W^i]]\}^n_{i=1}$. Node $H$ has states \(h_1,\ldots,h_n\) and prior $\theta'(h_i) = w_i$. Each node $Z \in \Z$ now has an extra parent $H$ in addition to its original parents in $G$. The new CPT of node $Z$ is set so that it reduces to its original CPT when $H = h_i$ for $Z \in G^i$. For details please refer to~\cite{huang2023algorithm}.
\end{enumerate}
\end{definition}
Let $\kappa$ be the set of auxiliary evidence created for syncing non-root unit variables $\U^c$. We then have $L(\u) = \pr'(\y, \w|\x, \v, \e, \kappa, \u)$ on $G'$. 
\haiying{For example\footnote{This example is created by ~\cite{huang2023algorithm}.}, consider a base model $G$ (Figure~\ref{fig:scm}) with causal objective function $L(u) = w_1 \cdot \pr(y_x, y'_{x'}|u) + w_2\cdot\pr(y_x, y_{x'}|u)$. Figure~\ref{fig:test} shows how to construct the corresponding objective model $G'$. The objective $L$ can then be evaluated as a single observational probability $\pr'([y^1], [[{y'}^1]], [y^2], [[y^2]] \mid [x^1], [[{x'}^1]], [x^2], [[{x'}^2]],u)$ on $G'$ (Figure~\ref{fig:objective}).
}


The correctness of the objective model has been studied in-depth~\cite{huang2023algorithm} and is not the focus of this work. We highlight that the problem finally amounts to optimizing a classical probability of the form $\max_{\u} \pr(\e_1|\u, \e_2)$ on the objective model, which can be larger and denser than the original SCM.

\paragraph{Reverse-MAP (R-MAP)} Consider an SCM $G$ and let $\U$, $\E_1$, $\E_2$ be disjoint \haiying{sets of variables} in $G$. The R-MAP problem is defined as \(\rmap(\U, \e_1, \e_2) \triangleq \argmax_{\u} \pr(\e_1|\u, \e_2)\) to be contrasted with the classical MAP problem, $\map(\U, \e) \triangleq \argmax_\u \pr(\u|\e)$ (or $\pr(\u, \e)$ equivalently). In the context of causal reasoning, MAP is concerned with finding the most likely outcome given a specific cause, while R-MAP is concerned with finding the most likely cause for a specific outcome (with the presence of other cause). They are different problems as discussed in~\cite{huang2023algorithm} and R-MAP captures the essence of unit selection better than MAP.

\cite{huang2023algorithm} shows how to adapt the classical variable elimination (VE) algorithm to solve R-MAP. Let $\V$ be the non-MAP variables. The basic idea is that we run two parallel VE in a synced way. In the first pass, we compute $\pr(\U, \e_1\e_2)$ by summing out $\V$ under evidence $\e_1\e_2$. In the second pass, we compute $\pr(\U, \e_2)$ by summing out $\V$ under evidence $\e_2$.~\cite{huang2023algorithm} shows that we can efficiently ``divide'' $\pr(\U, \e_1\e_2)$ and $\pr(\U, \e_2)$ to obtain $\pr(\e_1|\U,\e_2)$, if the two passes use the same elimination order.\footnote{The difficulty is that the space of $\U$ can be very large.} We finally compute the R-MAP probability by maxing out $\U$.




==> experiment.tex <==


We next apply the AC algorithm for R-MAP to solving unit selection problems on random SCMs, and compare its time and complexity to the VE algorithm for R-MAP --- VE\_RMAP in~\cite{huang2023algorithm}. Our algorithm, ACE\_RMAP, is implemented on top of the {\tt ACE} system\footnote{\url{http://reasoning.cs.ucla.edu/ace/}} which we use to compile the objective model into a decision-AC, and then evaluate the AC by the two-pass traversal as described in the previous section. The task is to find optimal units for the benefit function shown in Equation~\ref{eqn:benefit-ang}. The function has 4 counterfactual components with the same outcome variable $Y$ and action variable $X$.  We next describe the procedure used to generate problem instances.

\paragraph{Problem Generation} We generate random SCM $G$ according to the method in ~\cite{han2022on} and carefully choose unit variables $\U$, outcome variable $Y$, and action variable $X$ of the benefit function $L$ such that $\U, X, Y$ respect meaningful causal relationships. We first generate a DAG $G_0$ with $n$ binary nodes and a maximum number of parents $p$, which is used as the backbone of our SCM. We next add a node $Y$ as a child of the leaf nodes in $G_0$ and set $Y$ as outcome. We randomly choose a cause (ancestor) of $Y$ as action $X$. We then convert $G_0$ into SCM $G$ by adding a unique root parent for each internal node in $G_0$. The resulting $G$ tends to have many root nodes. This is meant to mimic the structure of SCMs commonly used for counterfactual reasoning.
We choose unit variables $\U$ by randomly picking 
50\% of the variables satisfying the following constraints: a unit variable $U$ must be a common cause (ancestor) of $X, Y$ and $U$ remains a cause (ancestor) of $Y$ after removing all edges incoming into $X$ in $G_0$.

For each problem instance $\langle G, \U, X, Y \rangle$, we construct an objective model $G'$ by composing triplet-models $G^1,\ldots, G^4,$ one for each component in the benefit function, as discussed earlier; see \cite{huang2023algorithm} for more details. We then run ACE\_RMAP on $G'$ to find the optimal units and compare its results against VE\_RMAP implemented in {\tt NumPy}. The computation for each instance is given 10 minutes to complete. For each problem instance, we report the execution time of ACE\_RMAP and VE\_RMAP. We also report the size of the circuit generated by ACE (ac\_size), and the total size of all factors generated by VE  (ve\_size), which are two comparable parameters that measure the total number of arithmetic operations required by ACE\_RMAP and VE\_RMAP, respectively. We also report the approximate constrained treewidth (tw) of $G'$, which is computed using minfill heuristics to find a constrained elimination order for VE\_RMAP; see~\cite{huang2023algorithm} for the need of a constrained order. 

\paragraph{Results} We used $n \in \{10, 15, 20, 25, 30, 35, 40, 45, 50\}$ and $p=6$ which results in SCM with $n'\simeq2n$ nodes and objective model with $\leq 12n$ nodes. For each $n$, we generate 25 instances and report the average statistics in Table~\ref{tab:benefit-function-exp}. We highlight the patterns from the statistics. First, as $n$ increases, the time and the number operations of  VE\_RMAP grows exponentially and becomes impractical after $n > 30$ (running out of memory\footnote{NumPy does not support ndarrays with $>32$ dimensions.}). This is predicted as VE\_RMAP is purely structure-based and must be exponential in the constrained treewidth (tw). Second, ACE\_RMAP is much more efficient than VE\_RMAP, leading to orders-of-magnitude speedups as a result of exploiting the high-degree of local (parameteric) structure in the objective model (e.g., 0/1 parameters, context-specific independence, parameter equality). This enables ACE\_RMAP to support very large and dense models (with $tw > 30$) that are normally out-of-reach if such parametric structure is not exploited.



==> intro2.tex <==
A theory of causality has emerged over the last few decades based on two parallel hierarchies, 
an {\em information hierarchy} and a {\em reasoning hierarchy,} often called the {\em causal hierarchy}~\cite{pearl18,Bareinboim20211OP}. 
On the reasoning side, this theory has crystallized three levels of reasoning with increased sophistication and proximity 
to human reasoning: associational, interventional and counterfactual, which are exemplified by the following canonical probabilities.
{\em Associational} \(\pr(y | x)\): probability of \(y\) given that \(x\) was observed (e.g., probability that a patient has a flu given they have a fever).
{\em Interventional} \(\pr(y_x)\): probability of \(y\) given 
that \(x\) was established by an intervention,
which is different from \(\pr(y | x)\) (e.g.,
seeing the barometer 
fall tells us about the weather but moving the barometer needle won't bring rain).
{\em Counterfactual} \(\pr(y_x | y', x')\): probability of \(y\) if we were to establish
\(x\) by an intervention given that neither \(x\) nor \(y\) are true (e.g., probability that a patient who
did not take a vaccine and died would have recovered had they been vaccinated).
On the information side, these forms of reasoning 
require different
levels of knowledge, encoded as associational, causal and functional (mechanistic) models, 
with each class of models containing more information than the preceding one. In the framework of probabilistic graphical models
\cite{PGMbook}, such knowledge is encoded 
by Bayesian networks~\cite{Pearl88b,DarwicheBook09}, 
causal Bayesian networks~\cite{pearl00b,PetersBook,SpirtesBook} and functional Bayesian networks~\cite{uai/BalkeP95}
also called {\em structural causal models} (SCMs)~\cite{halpern2000axiomatizing}.

The \textit{unit selection problem} emerged from this theory of causality and has been receiving attention as it provides a rigorous framework to analyze and optimize the causal behavior of objects (e.g., agents). 
% It was initially proposed by~\cite{ijcai/LiP19} who motivated it using the problem of selecting customers to target by an encouragement offer for renewing a subscription. 
% The unit selection problem is based on a \textit{causal objective function} which mentions a special set of variables $\U$, called \textit{unit variables,} and can include any quantities from the causal hierarchy: associational, interventional, or counterfactual. The goal of this problem is to find an instantiation $\u$ of unit variables which optimizes the given objective function. Intuitively, this is meant to identify units ($\u$), which can be individuals or arbitrary objects such as policies, based on their causal behavior. 
\haiying{
    It was initially proposed by~\cite{ijcai/LiP19} who motivated it using the problem of selecting customers to target who would renew a subscription if an enticement is offered. This problem is challenging in two senses: first, the prediction of counterfactual behavior --- how an individual would act under a hypothetical scenario that is not directly observable. For example, when we observe a customer renew a subscription with a discount, we don't know whether they would have done the same if this discount were not offered. %and when we observe a customer leaves without a discount, we don't know whether they would decide to leave regardless of this discount. 
    Second,  the large space of customer characteristics (age, income, purchase history, etc) so that optimization over this space poses a scalability problem. 
    % For example, when a company launches a new product, it may not yet gather sufficient data for each combination of characteristics. 
    To identify customers of interest, a {\em benefit function} is proposed in~\cite{ijcai/LiP19} that characterizes customers as responders, always-takers, deniers and contrarians, which is a special case of {\em causal objective functions}. A causal objective function mentions a special set of variables $\U$, called \textit{unit variables,} and can include any quantities from the causal hierarchy: associational, interventional or counterfactual. The unit selection problem is to find an instantiation of unit variables (called units $\u$) which optimizes the given objective function.
    In ~\cite{huang2023algorithm} a more general class of causal objective functions was introduced to identify structured units, which can be individuals or arbitrary objects (e.g., decisions, policies, activities) in broader contexts beyond the customer targeting scenario.
 }

Unit selection embeds two subproblems that are hard in general: {\em evaluation} and {\em optimization} of the objective function~\cite{ijcai/LiP19}. Prior work focused on the evaluation problem, which is concerned with estimating the value of a causal objective function using observational and experimental data given a non-parametric causal graph. This stems from the identifiability problem, which has been extensively studied by the causality community. Useful bounds and criteria have been derived for this purpose with respect to the specific benefit function~\cite{ijcai/LiP19,li2022unit_ab,aaai/LiP22,corr/LiP22a,li2022unit}.

A recent work~\cite{huang2023algorithm} investigated the optimization problem: finding units that maximize the score defined by the causal objective function---assuming a fully specified SCM so as to obtain point-values for the objective function. They first show that a broad class of causal objective functions can be reduced to an associational probability on a meta-model, called the \textit{objective model.} They
also showed that optimizing this (surrogate) probability requires solving a variant of the Maximum A Posteriori (MAP) inference problem, called \textit{Reverse-MAP (R-MAP).} They further showed how to modify the classical Variable Elimination (VE) algorithm to solve R-MAP. This treatment, in principle, would allow us to find the exact optimal units. However, computing R-MAP on the objective model remains a hard task---in fact, it is $\NP^{\PP}$-complete as shown in~\cite{huang2023algorithm}. In practice, the objective model is usually much larger and denser than the original SCM. Moreover, running VE on the objective model must be exponential in its constrained treewidth~\cite{jair/ParkD04}, and can  also be exponential in the number of unit variables depending on the form of the specific objective function. 

We address this computational challenge by introducing a new method for solving R-MAP on a model $G$ by compiling $G$ into a tractable arithmetic circuit (AC)~\cite{Darwiche03,faia/Darwiche21} and computing R-MAP on the circuit in linear time. Using ACs for inference allows us to exploit the local/parametric structure of a model which means that we may be able to handle models that are out of reach of classical, structure-based inference algorithms like VE; see, e.g.,~\cite{Chavira.Darwiche.Ijcai.2005,ChaviraDJ06,Chavira.Darwiche.Aij.2008}. And this is indeed what our empirical evaluation shows.

\shrink{
In particular, we show that if an arithmetic circuit (AC) that represents a distribution $\pr$ satisfies certain constraints known as {\em marginal determinism}, then the circuit can be modified to compute R-MAP probabilities with respect to $\pr$ in time linear in the circuit size, similar to how variable elimination for MAP is modified to compute R-MAP.}


This paper is structured as follows. We start by a review of the unit selection problem and its reduction to R-MAP. We then provide some background on ACs and how they can be used to solve MAP in time linear in the AC size. We follow by our proposed linear-time method for solving R-MAP on ACs, and a corresponding empirical evaluation which shows orders-of-magnitude speedups compared to the state-of-the-art. We finally close with some concluding remarks.
